Results and Insights from Diagnostic Questions: The NeurIPS 2020 Education Challenge

This competition concerns educational diagnostic questions, which are pedagogically effective, multiple-choice questions (MCQs) whose distractors embody misconceptions. With a large and ever-increasing number of such questions, it becomes overwhelming for teachers to know which questions are the best ones to use for their students. We thus seek to answer the following question: how can we use data on hundreds of millions of answers to MCQs to drive automatic personalized learning in large-scale learning scenarios where manual personalization is infeasible? Success in using MCQ data at scale helps build more intelligent, personalized learning platforms that ultimately improve the quality of education en masse. To this end, we introduce a new, large-scale, real-world dataset and formulate 4 data mining tasks on MCQs that mimic real learning scenarios and target various aspects of the above question in a competition setting at NeurIPS 2020. We report on our NeurIPS competition in which nearly 400 teams submitted approximately 4000 submissions, with encouragingly diverse and effective approaches to each of our tasks.

==> metrics.tex <==

\iffalse
\section{Metrics}

The metrics for each task are as follows:
\begin{enumerate}
    \item \textbf{Task 1:} Prediction accuracy $A$ -- the number of predictions that match the true correctness indicator, divided by the total number of predictions (in the held-out test set): 
    $A = \frac{N_{correct\_predictions}}{N_{total\_predictions}}$.
    
    \item \textbf{Task 2:} Prediction accuracy as above, except that the true answers are now categorical instead of binary.
    
    \item \textbf{Task 3:} The participants will submit a quality ranking for the questions (Figure \ref{fig:task3metric} \textit{Left}). An unseen set of question-pairs will then be used to evaluate the quality of this ranking (and thus the underlying metric). Note that we have collected the experts' judgement of which question in each pair is of higher quality. The evaluation steps are then as follows (see also Figure \ref{fig:task3metric} \textit{Right} for an illustration):
    \begin{itemize}
        \item Determine, based on the submitted ranking, which question in each pair is of higher quality.
        \item Compare this with each expert's judgement (assign 1 if matching, 0 if not matching).
        \item For each expert $i$, determine the agreement fraction: $A_i = \frac{N_{matching\_pairs}}{N_{total\_pairs}}$ .
        \item Find the \textit{maximum} of these agreement fractions $A_{max} = \max_{i} A_i$. This will be used as the final evaluation metric for this task.
    \end{itemize}
    
    We are using looking for metrics that can approximate \textit{an} expert judgement really well, hence we use the maximum of the agreement fractions, rather than a mean of the agreement fractions over all experts. The reasoning for this approach is that the quality metrics of the experts are in themselves subjective, and it is interesting to find whether a particular expert's approach can be approximated especially well by the use of machine learning. \al{Double check we are actually reporting the mean afterwards} Note that we will report the mean of the agreement fractions metric at the end of the competition, but this will not be used to judge the task winner.

    \item \textbf{Task 4: } Submitted models will be asked to sequentially choose 10 query questions for each student in a held-out set of students, with the answer to each question revealed to the model in private after selection. The model is given the opportunity to incorporate this information or retrain after the response to each question is revealed. After receiving 10 answers for each student, the model will be assessed on its prediction accuracy on a held-out test set of answers for each of these students, that cannot be queried. \al{current scoring setup just uses binary data} As in Task 1, binary data will be used for this task.

%\[\textrm{MRR} = \frac{1}{|\mathcal{S}|}\sum_{i=1}^{|\mathcal{S}|}\frac{1}{\textrm{rank}_i}\]
\end{enumerate}

\fi

==> protocol.tex <==
\section{Submission Protocol}
\label{sec:submission}

Each task in the competition contains two phases: a public evaluation phase and a private evaluation phase. Results in the public evaluation phase are displayed on a public leaderboard allowing participants to see how their submissions perform compared to other participants. Results in the private evaluation phase are hidden until the end of the competition. \textbf{Important: For each task, participants must submit to both the public and private evaluation phases separately. Submissions made solely to the public evaluation phase will not be used in the final judging of the competition. It is the participants' responsibility to make sure their submission to the private phase of each task represent their best results.} For tasks 1-3, submission template files are provided for both the public and private phases, which must be submitted to CodaLab. For task 4, a participants model must be submitted to both the public and private leaderboards, where it will be evaluated separately.

Before submission, the participants must first zip their submission files into one zip file. CodaLab only accepts one single \texttt{.zip} file as the submission file. 
The submission buttons are under \texttt{Participate} tab on the top of the competition website and under the \texttt{Submit/View Results} tab on the left. The tabs on the top of this page, e.g., \texttt{Task 1 Public}, contains the submission link to each of the tasks.

Below are the detailed submission instructions for each task.

\subsection{Submission for Tasks 1-3}
The first three tasks are evaluated through the submission of a zipped CSV file to Codalab:
\noindent
\begin{itemize}
    \item \textbf{Task 1}: Participants are provided with a CSV file (in the folder \texttt{starter\_kit/submission\_templates}) containing (UserId, QuestionId) pairs for which the answer is unseen. They must fill in their prediction for whether the student will answer the question correctly in each case. 
    {\bf Important: the submission file must be a \texttt{.zip} file containing a file named \texttt{submission\_task\_1.csv}}.
    \item \textbf{Task 2}: Participants are provided with a CSV file (in the folder \texttt{starter\_kit/submission\_templates}) containing (UserId, QuestionId) pairs for which the answer is unseen. They must fill in their prediction for which answer the student will give to the question in each case. 
    {\bf Important: the submission file must be a \texttt{.zip} file containing a file named \texttt{submission\_task\_2.csv}}.
    \item \textbf{Task 3}: Participants are provided with a CSV file (in the folder \texttt{starter\_kit/submission\_templates}) containing a list of all of the QuestionIds provided in the dataset for Task 3. They are asked to fill in a 'Ranking' column indicating the rank (1-948) they give to each question, where 1 is the highest-quality question and 948 is the lowest-quality question.
    {\bf Important: the submission file must be a \texttt{.zip} file containing a file named \texttt{submission\_task\_3.csv}}.
\end{itemize}
\subsection{Submission for Task 4}\label{task_4_submission}
Task 4 is evaluated through a code submission. Participants are provided with a template file \texttt{submission\_model\_task\_4.py}, which provides a simple API wrapper through which the evaluation script will interface with submitted models. The methods which participant must implement are as follows:
\begin{itemize}
    \item \textbf{\_\_init\_\_}: Load a participant's model from this file or a neighbouring file (e.g. a separate \texttt{model.py} file where the model is defined) and perform any initialisation that is required.
    \item \textbf{select\_questions}: Select the next question to query for each question, given the data observed by the model so far (both the binary correctness indicators and the specific multiple-choice answers) and an array indicating which questions can be queried for each student.
    \item \textbf{update\_model}: Optionally update the model based on the new data revealed after revealing new answers.
    \item \textbf{predict}: Predict a binary correctness indicator for each student, for all questions for which we have not observed the student's answer.
\end{itemize}

Details of the specific signatures of these functions can be found in the template \texttt{submission\_model\_task\_4.py} file. The evaluation procedure is as follows:
\begin{enumerate}
    \item Initialise the model with \texttt{\_\_init\_\_()}.
\item For 10 steps, first select a new feature with \texttt{select\_questions()}, reveal the selected values, and pass the new data to \texttt{update\_model()}.
\item After 10 feature selection steps, call \texttt{predict()} to make binary predictions for the held-out target elements and evaluate the model's prediction accuracy.
\end{enumerate}

The submission files for this task must contain \texttt{submission\_model\_task\_4.py}.
Users are free to include additional files, such as model definitions or trained model weights, in their submissions.
To submit, the \texttt{submission\_model\_task\_4.py} template file and any additional files should be zipped into one single \texttt{.zip} file and then submitted to CodaLab. 
{\bf Important: please \textit{do not} change the class method names in \texttt{submission\_model\_task\_4.py}. Also, for any saved model files, participants \textit{must} use \texttt{model\_task\_4\_} as the prefix of the file name for submission}. For example, if the model is called \texttt{my\_pytorch.pt}, then for submission , this model file must be renamed to \texttt{model\_task\_4\_my\_pytorch.pt}.

During evaluation, all training data and metadata files included as part of task 4 will be added to the root of the submission directory, 
and submissions may make use of these files as they wish. Simply specifying the name of the dataset to load should be sufficient to load the files -- for instance, the training data can be accessed by submitted models at the path ``\texttt{./train\_task\_3\_4.csv}''. Note that users are expected to upload a trained model for submission, as time limits on the submission compute workers will likely render training prior to evaluation too time-consuming.

For each task, there is a daily and total submission limit specified on the relevant submission page on Codalab.  Unsuccessful submissions due to errors will not count against this total. \textbf{Submissions must be made separately to both the public and private components of the leaderboard}, with the final competition results being based solely on the private leaderboard.

\subsection{Leaderboard}
The submitted result will show up in a public leaderboard for each public phase of the competition. The public leaderboard shows how the participant(s) stand against other participants on the public evaluation data for each task. 

Note that the leaderboard only shows the same ``score'' column for all tasks; participants should be aware that the meaning of the ``score'' is different for each task; please refer to the details of the evaluation metrics for each task in Section~\ref{sec:tasks}. Nevertheless, a more detailed result can be accessed in the ``detailed results'' part on the rightmost column of the table under the ``Results'' tab of the competition website.

For all private phases of the competition, no public leaderboard will be shown and results are only visible by the competition organizers.

\subsection{Computation Environment}
The evaluation on CodaLab is performed using the an off-the-shelf docker image that contains most of the data science, machine learning and deep learning packages. Participants must ensure that their submissions are able to run in this environment. Please see \url{https://github.com/ufoym/deepo} for more detail.

==> rules.tex <==
% \section{Rules}
% \CZ{We can put this to the last section. They are much less important than the getting started section}
% \al{Need to review these, they're old}

% \noindent

% The rules of the competition are as follows: 
% \begin{itemize}
% \item Users may work in teams of up to 10 people. 
% \item In tasks that require a code submission to be executed, entrant's code must run on the provided compute environment within 1 hour. This is to encourage computationally efficient solutions appropriate for real-time personalized education.
% \item During the evaluation of the submitted code, the individual containers will not have access to any external network to avoid any information leak.
% \item The submitted code must generate predictions using a machine learning model. Submissions making hard-coded predictions are forbidden.
% \item Users may make use of open source libraries given proper attribution. At the end of the competition, we encourage all code to be open-sourced so the results can be reproduced. 
% \item The use of supplementary existing open-source datasets for e.g. pre-training is permitted provided they are credited. The use of private, proprietary datasets is not permitted.
% \item The questions images have been shared solely for the purpose of this competition and must not be used for any other purpose. The question images must not printed or shared with anyone outside of the competition.
% \item Any parties or individuals affiliated with Eedi, Microsoft Research or the Computational and Biological Learning Group, University of Cambridge are not eligible for the prizes, but may participate in the competition.
% \item For participants to be eligible for prizes their code must be publicly available. 
% \item Any instances of cheating, defined as violation of the rules above or any other attempt to circumvent the spirit and intent of the competition, as determined by the organizers, will result in the invalidation of all of the offending team's submissions and a disqualification from the competition.
% \end{itemize}


% In order to prevent cheating, all the evaluation data will be kept completely inaccessible to the participants during the competition. The aforementioned rules on manual review of the submissions and lack of network access during code evaluation also aim to prevent cheating.

==> starting.tex <==
\section{Getting Started: Sample Model, Local Evaluation and Submission Preparation}
\label{sec:get-started}


\subsection{Quick Start}

Both the public data and starter kit for the competition can be found under the tab \texttt{Participate}/\texttt{Get Data}/ from the competition homepage. The starter kit contains a number of utility scripts and sample models to allow easy participation in the competition. Submission templates for preparing submissions in the correct format for each task are included in the \texttt{submission\_templates} directory.

To quickly get started with the competition, follow these instructions:
\begin{enumerate}
   \item Download the training data and starter kit from the competition homepage.
   \item Place the downloaded \texttt{data} directory into the root of the \texttt{starter\_kit} directory.
   \item (Optional) Run the \texttt{local\_data\_split.py} files for each task in order to generate validation sets for local model evaluation.
   \item Run the sample model files provided for tasks 1-3 in order to generate sample submissions for the competition. Task 4 requires no generation, as participants must submit the model code itself.
\end{enumerate}

To submit solutions to Tasks 1-3, participants should submit a \texttt{.zip} file containing a completed submission template file named \texttt{submission\_task\_n.csv} where \texttt{n} is the task number. This file should then be uploaded to \textbf{both} the public and private phases of the appropriate task.

To submit solutions to Task 4, participants should submit a \texttt{.zip} file containing a completed submission API wrapper file \texttt{submission\_model\_task\_4.py}, in additional to any additional model files or artifacts required in order to run the trained model.

Each task has its own self-contained directory, which typically includes a script for creating a local ``validation set'' for local model evaluation, a script for performing local model evaluation, and an example model to help get started with the task.

Further details for each task's resources are provided in the following sections.

\subsection{Task 1}
\paragraph{Available Files} The following files are available for Task 1:
\begin{itemize}
    \item Training data: \texttt{train\_task\_1\_2.csv}, in the folder \texttt{data/train\_data}
    \item Submission template: \texttt{submission\_task\_1\_2.csv}, in the folder \\ \texttt{starter\_kit/submission\_templates}
     \item Question metadata: \texttt{question\_metadata\_task\_1\_2.csv}, in the folder  \texttt{data/metadata}
    \item Student metadata: \texttt{student\_metadata\_task\_1\_2.csv}, in the folder  \texttt{data/metadata}
    \item Answer metadata: \texttt{answer\_metadata\_task\_1\_2.csv}, in the folder  \texttt{data/metadata}
    \item Local evaluation scripts: \texttt{local\_data\_split.py}, \texttt{local\_evaluation.py}, in the folder\\ \texttt{starter\_kit/task\_1}
    \item Sample baseline model: \texttt{sample\_model\_majority.py}, in the folder \texttt{starter\_kit/task\_1}
\end{itemize}


\paragraph{Submission to CodaLab}
To submit to CodaLab, participants must submit results containing predictions for {\it each and every} \texttt{(UserId, QuestionId)} pair in the submission template file \texttt{submission\_task\_1\_2.csv}. Running the provided \texttt{sample\_model\_majority.py} script will generate an example of this file, creating a directory \texttt{../submissions} by default where the generated file is named as \texttt{submission\_task\_1.csv} which is ready to be zipped and submitted.

{\bf Important}: make sure the name of the prediction column in submissions is \texttt{IsCorrect}. 

\paragraph{Local Evaluation} 

To evaluate locally on a validation set produced from the training data, follow the steps below:
\begin{enumerate}
    \item Navigate into the folder \texttt{starter\_kit/task\_1}
    \item Split the data. We have provided a script \texttt{local\_data\_split.py} to do so; participants can perform data split by running \\
    \centerline{\texttt{python local\_data\_split.py}}\\ which generates a train and validation set using the training data. By default, the split files are named as \texttt{train\_task\_1\_2.csv} and \texttt{valid\_task\_1\_2.csv} and are saved in the folder \texttt{data/test\_input}.
    \item Run your model and make predictions. We have provided a sample model \\ \texttt{sample\_model\_majority.py} to help get started. Note that in order to run this model on the local evaluation data split, the block of code marked ``Default arguments for Codalab submission" should be commented out, and the block marked ``Default arguments for local evaluation" should be uncommented. To get predictions using this model, please run \\
    \centerline{\texttt{python sample\_model\_majority.py}} \\ This model outputs a \texttt{.csv} file containing the results at \\(\texttt{data/test\_input/test\_submission\_task\_1.csv}).
    \item Evaluation. Run \\
    \centerline{\texttt{python local\_evaluation.py} }\\with appropriate options; see \texttt{argparse} arguments. This command computes and saves the score using the prediction and validation set. A score and confusion matrix are saved to the  \texttt{output\_dir} which by default is \texttt{data/test\_output}. The official evaluation for this task implements the same evaluation metric as that in \texttt{local\_evaluation.py}.
\end{enumerate}


\subsection{Task 2} 
\paragraph{Available Files}
The following files are available for Task 2:
\begin{itemize}
    \item Training data: \texttt{train\_task\_1\_2.csv}, in the folder \texttt{data/train\_data}
    \item Submission template: \texttt{submission\_task\_1\_2.csv}, in the folder\\ \texttt{starter\_kit/submission\_templates}
    \item Question metadata: \texttt{question\_metadata\_task\_1\_2.csv}, in the folder  \texttt{data/metadata}
    \item Student metadata: \texttt{student\_metadata\_task\_1\_2.csv}, in the folder  \texttt{data/metadata}
    \item Answer metadata: \texttt{answer\_metadata\_task\_1\_2.csv}, in the folder  \texttt{data/metadata}
    \item Subject metadata: \texttt{subject\_metadata.csv}, in the folder  \texttt{data/metadata}
    \item Local evaluation scripts: \texttt{local\_data\_split.py}, \texttt{local\_evaluation.py}, in the folder \\\texttt{starter\_kit/task\_2}
    \item Sample baseline model:  \texttt{sample\_model\_majority.py}, in the folder \texttt{task\_2}
\end{itemize}
\paragraph{Local Evaluation and Prepare Submission}
Since Task 2 is very similar in nature to Task 1, the training data and submission templates are the same and the local evaluation scripts are similar. The only difference is that Task 2 predicts the actual response that a student makes to a question (answer A, B, C or D to each multiple-choice question, encoded as 1, 2, 3 or 4 respectively).

{\bf Important}: make sure the name of the prediction column in the submission file is \texttt{AnswerValue}.

\subsection{Task 3}
\paragraph{Available Files}
The following files are available for Task 3: 
\begin{itemize}
    \item Training data: \texttt{train\_task\_3\_4.csv}, in the folder \texttt{data/train\_data}
    \item Submission template: \texttt{submission\_task\_3.csv}, in the folder \\ \texttt{starter\_kit/submission\_templates}
    \item Question images: in the folder \texttt{data/images/}
    \item Question metadata: \texttt{question\_metadata\_task\_3\_4.csv}, in the folder  \texttt{data/metadata}
    \item Student metadata: \texttt{student\_metadata\_task\_3\_4.csv}, in the folder  \texttt{data/metadata}
    \item Answer metadata: \texttt{answer\_metadata\_task\_3\_4.csv}, in the folder  \texttt{data/metadata}
    \item Subject metadata: \texttt{subject\_metadata.csv}, in the folder  \texttt{data/metadata}
    \item Sample baseline model: \texttt{sample\_model\_entropy.py}, in the folder \texttt{starter\_kit/task\_3}

\end{itemize}

\paragraph{Submission to CodaLab}
This task asks participants to rank the quality of questions in the training data \texttt{train\_task\_3\_4.csv} in descending order, i.e., rank 1 represents the highest quality, rank 2 represents the second highest quality, etc. There is no ground-truth provided and local evaluation is not possible; rather, we provide a baseline model which ranks the questions based on an estimation of their entropy (\texttt{sample\_model\_entropy.py}) to generate results appropriate for submission for Task 3. See the implementation in this files for details of the computations. The submission file contains 2 columns \texttt{(QuestionId, ranking)} where the second column is the ranking for each question. Each question should have a unique ranking, i.e., no two rankings should be the same. 

The training data and metadata provided for tasks 3 and 4 is in the same format as that of tasks 1 and 2, but uses a disjoint, smaller set of questions. As explained in section \ref{sec:data}, the randomized IDs used in Tasks 1 and 2 are generated independently of those used in Tasks 3 and 4, and so participants should not attempt to use the data from Tasks 1 and 2 to aid them in Tasks 3 and 4.

To prepare submission run your model which generates the ranking for all question IDs in the \texttt{submission\_task\_3.csv} file. The provided entropy-based model demonstrates this process; simply run\\
 \centerline{\texttt{python sample\_model\_random.py}}\\
This will create a prediction file \texttt{test\_submission\_task\_3.csv} in the \texttt{../submissions} folder by default. This file is ready to be zipped and submitted.

{\bf Important}: the ranking column must be named \texttt{ranking} for the CodaLab evaluation script to correct read the participants' predicted quality rankings.

\subsection{Task 4}
\paragraph{Available Files}
The following files are available for Task 4:
\begin{itemize}
    \item Training data: \texttt{train\_task\_3\_4.csv}, in the folder \texttt{data/train\_data}
    \item Submission template file: \texttt{submission\_task\_4.py}, in the folder \texttt{submission\_templates}
    \item Question images: in the folder \texttt{data/images/}
    \item Question metadata: \texttt{question\_metadata\_task\_3\_4.csv}, in the folder  \texttt{data/metadata}
    \item Student metadata: \texttt{student\_metadata\_task\_3\_4.csv}, in the folder  \texttt{data/metadata}
    \item Answer metadata: \texttt{answer\_metadata\_task\_3\_4.csv}, in the folder  \texttt{data/metadata}
    \item Subject metadata: \texttt{subject\_metadata.csv}, in the folder  \texttt{data/metadata}
    \item Local evaluation scripts and models: 
    \vspace{-5pt}
    \begin{itemize}
        \item \texttt{local\_data\_split.py} is in the folder \texttt{starter\_kit/task\_4} 
        \item \texttt{local\_evaluation.py}, \texttt{train\_model.py}, \texttt{submission\_model\_task\_4.py},\\ \texttt{model\_task\_4.pt}, \texttt{model.py} in the folder \texttt{starter\_kit/task\_4/pytorch}
         \item \texttt{local\_evaluation.py}, \texttt{train\_model.py}, \texttt{submission\_model\_task\_4.py},\\ \texttt{model\_task\_4\_most\_popular.npy}, \texttt{model\_task\_4\_num\_answers.npy}\\
         \texttt{model.py}, in the folder \texttt{starter\_kit/task\_4/numpy}
    \end{itemize}

\end{itemize}

\paragraph{Submission to CodaLab}
As detailed in \nameref{task_4_submission}, participants should submit to CodaLab a \texttt{.zip} file containing their completed \texttt{submission\_model\_task\_4.py} file along with any supplementary model code or weights, where it will be evaluated in private. Submissions may assume that all training data and metadata files for the task will be included same directory as the submission files (i.e., \texttt{./}).


We have provided sample models and script to generate a sample submission ready for CodaLab. To do so, please follow the steps below:
\begin{enumerate}
    \item Navigate to either \texttt{starter\_kit/task\_4/numpy} or \texttt{starter\_kit/task\_4/pytorch}
    \item Run \\\centerline{\texttt{python train\_model.py}}\\
    which saves a model file to either the NumPy or PyTorch folder.
    \item If using the NumPy model, zip \texttt{model.py}, \texttt{submission\_model\_task\_4.py}, \texttt{model\_task\_4\_\\most\_popular.npy} and \texttt{model\_task\_4\_num\_answers.npy} to a \texttt{.zip} file. If using the PyTorch model, zip \texttt{model.py}, \texttt{submission\_model\_task\_4.py} and \texttt{model\_task\_4.pt} into a \texttt{.zip} file. Details on the naming of the files and what can be changed inside the submission template file \texttt{submission\_model\_task\_4.py} are discussed in Section~\ref{task_4_submission}.
\end{enumerate}

\paragraph{Local Evaluation}
In the starter kit for Task 4, a mock test environment is provided as part of the competition API, in order to allow the entrants to check that their submission will work with the evaluation procedure. Both the NumPy and PyTorch models described above can be evaluated locally in this way.
\begin{enumerate}
    \item Navigate into the folder \texttt{starter\_kit/task\_4}
    \item Split the data. We have provide a script \texttt{local\_data\_split.py} to do so; participants can perform data split by running \\
    \centerline{\texttt{python local\_data\_split.py}}\\ which generates a train and validation set using the training data. By default, the split files are named as \texttt{train\_task\_4.csv} and \texttt{valid\_task\_4.csv} and are saved in the folder \texttt{data/test\_input}.
    \item Train your model. We have provided a sample model file and training scripts using both NumPy and PyTorch. To train the sample models, navigate to either \texttt{starter\_kit/\\task\_4/numpy} or \texttt{starter\_kit/task\_4/pytorch} and run \\ \centerline{\texttt{python train\_model.py}}\\
    Note that in the NumPy model, the path to the training data in the \texttt{train\_model()} method will need to updated to point to the newly created ``local test" split.
    This script will save a model file to the NumPy or PyTorch folders above; see the \texttt{train\_model.py} script for more details. Note that the provided PyTorch model class does not implement a method to train the model; 
    \item Evaluate. Run \\
    \centerline{\texttt{python local\_evaluation.py} }\\ This command computes and prints the sequence of selected questions and the final accuracy.
\end{enumerate}


